History Determinism vs. Good for Gameness in Quantitative Automata

Automata models between determinism and nondeterminism/alternations can retain some of the algorithmic properties of deterministic automata while enjoying some of the expressiveness and succinctness of nondeterminism. We study three closely related such models -- history determinism, good for gameness and determinisability by pruning -- on quantitative automata. While in the Boolean setting, history determinism and good for gameness coincide, we show that this is no longer the case in the quantitative setting: good for gameness is broader than history determinism, and coincides with a relaxed version of it, defined with respect to thresholds. We further identify criteria in which history determinism, which is generally broader than determinisability by pruning, coincides with it, which we then apply to typical quantitative automata types. As a key application of good for games and history deterministic automata is synthesis, we clarify the relationship between the two notions and various quantitative synthesis problems. We show that good-for-games automata are central for "global" (classical) synthesis, while "local" (good-enough) synthesis reduces to deciding whether a nondeterministic automaton is history deterministic.

==> decidingGFG.tex <==
%\section{Deciding GFGness of LimSup automata}

The winner of the letter game is difficult to decide directly, as LimSup automata are not determinisable. We therefore generalise the token-game approach, introduced by Bagnol and Kuperberg~\cite{BK18}, to LimSup automata. As the absolute weights on the transitions of a LimSup automaton have no meaning, but only their relative order does, we assume the weights to be $\{1, 2, \ldots\}$.

\paragraph*{Token games} In the \textit{two token game}, known as $G_2$, the players proceed as in Eve's letter game, except that now Adam has two tokens that he must move after Eve has made her move, thus building two runs. One of these must witness a good run over the word Adam played. In the boolean setting, this run must be accepting, thus witnessing that the word is in the language of the automaton.
Here, the maximal value produced by Adam's runs witnesses a lower bound on the value of the word, and Eve's task is to match or surpass this value on her run.

In the boolean setting, $G_2$ has the same winner as the letter game, at least for B\"uchi~\cite{BK18} and coB\"uchi~\cite{BKLS20} automata (the parity case is, for now, open). Since $G_2$ is solvable in polynomial time for B\"uchi and coB\"uchi acceptance conditions, this gives a {\sc PTime} algorithm for deciding GFGness, which avoids the determinisation and complementation required for solving the letter game directly.

Here, we use a quantitative version of $G_2$ to show that the GFGness fo LimSup automata is decidable in quasipolynomial time.

\begin{definition}[$k$-token games]\label{def:G2}
A configuration of the game $G_k(\A)$ for $k\geq 1$ is a tuple $(\sigma, q, p_1,\dots p_k)$ where $q, p_1,\ldots, p_k \in Q$ are states and $\sigma\in\Sigma\cup\{\epsilon\}$ is a letter.
A play begins in $(\sigma_0,q_0, p_{1,0},\dots, p_{k,0})=(\epsilon,\iota, \iota,\dots, \iota)$ and consists of an infinite sequence of configurations $(\sigma_0,q_0,p_{1,0},\dots , p_{k,0})(\sigma_1,q_1, p_{1,1},\dots, p_{k,1})\ldots$. 
In a configuration $(\sigma_i,q_i,p_{1,i},\ldots, p_{k,i})$, the game proceeds to the next configuration $(\sigma_{i+1},q_{i+1},p_{1,i+1},\ldots,p_{k,i+1})$ as follows.  
\begin{itemize}
\item Adam picks a letter $a$ from $\Sigma$,
\item Eve picks a transition $q_{i}\xrightarrow{a} q_{i+1}$, and
\item Adam picks transitions, $p_{1,i}\xrightarrow{a} p_{1,i+1}, \dots, p_{k,i}\xrightarrow{a} p_{k,i+1}$
\end{itemize}
In the limit, a play consists of an infinite word $w$ that is derived from the concatenation of $\sigma_0,\sigma_1,\ldots$, as well as $k+1$ infinite sequences $\pi$ (picked by Eve) and  $\pi_1\dots \pi_k$ (picked by Adam) of transitions over $w$. Eve wins the play if $\Val(\pi) \geq  \max(\Val(\pi_1),\dots, \Val(\pi_k))$.

\end{definition}

We now observe that $G_2(\A)$, for a LimSup automaton $\A$, can be solved via a reduction to a parity game.

\begin{lemma}\label{lem:solveG2}
Given a nondeterministic LimSup automaton $\A$, the game $G_2(\A)$ can be solved in quasipolynomial time with respect to the size of $\A$. For automata with a fixed number of weights, it can be solved in polynomial time  with respect to the size of $\A$. 
\end{lemma}

\begin{proof}
We encode the game $G_2(\A)$, for a LimSup automaton $\A=(\Sigma,Q,\iota,\delta,\gamma)$, into a parity game as follows.

The positions are tuples $(\sigma,q,p,p',m)\in \Sigma\cup \varepsilon \times Q^3\times \{l,e,a\}$ consisting of a possibly empty letter representing the last letter played, three states of $\A$ to represent the current state of each player's run(s), and a variable in $\{l,e,a\}$ indicating whether it is Adam's turn to play a letter, Eve's turn to pick a transition, or Adam's turn to pick two transitions, respectively.

The moves are:
\begin{itemize}
\item from $(\varepsilon,q,p,p',l)$ to $(\sigma,q,p_1,p_2,e)$ for each $\sigma\in \Sigma$. Such moves have priority $0$.
\item from $(\sigma,q,p_1,p_2,e)$ to $(\sigma, q', p_1,p_2, a)$ for all $q'$ such that there is a transition $t=q\xrightarrow{\sigma} q'$. The priority of such a move is $2\gamma(t)$.
\item  from $(\sigma,q,p_1,p_2,a)$ to $(\varepsilon, q, p_1',p_2',l)$ for all $p_1'$ and $p_2'$ such that there are transitions $t_1=p_1\xrightarrow{\sigma}p_1'$ and $t_2=p_2\xrightarrow{\sigma} p_2'$. The priority of such a move is $2\max(\gamma(t_1), \gamma(t_2))-1$.
\end{itemize}

Positions $(\sigma,q,p_1,p_2,m)$ belong to Adam if $m\in \{l,a\}$ and to Eve otherwise. The parity game begins from $(\varepsilon, \iota,\iota,\iota,l)$.

We claim that Eve wins this parity game if and only if she wins $G_2(\A)$. It should be clear that the moves of the parity game correctly encode the moves in the letter game, so there is a bijection between plays in $G_2(\A)$ and plays of the parity game. It therefore remains to argue that the priorities correctly encode the winner of $G_2(\A)$. Indeed, observe that the even priorities seen infinitely often in a play of the parity game are exactly priorities $2x$, where $x$ is a weight seen infinitely often in Eve's run in the coresponding play in $G_2(\A)$. The odd priorities seen infinitely often on the other hand are $2x-1$, where $x>0$ occurs infinitely often on one of Adam's runs in the corresponding play of $G_2(\A)$. Hence, Eve can match the maximal value of Adam's runs in $G_2(\A)$ if and only if she can win the parity game encoding $G_2(\A)$.


This parity game is of size polynomial in the size of $\A$; the number of priorities is linear in the number of weights in $\A$. It can then be solved in quasipolynomial time, or in polynomial time if the number of priorities is fixed, using the reader's favourite quasipolynomial parity game algorithm, for instance~\cite{CJKLS17}.
\end{proof}

\begin{remark}\label{rem:positionalGk}
Observe that the same reduction works for the $k$-token game $G_k(\A)$, for every $k$, and the positions of the parity game and the $k$-token game are isomorphic. Therefore, whenever Eve wins in some $k$-token game on a LimSup automaton, she wins it with a positional strategy.
\end{remark}

The rest of the section is dedicated to proving that $G_2$ characterises GFGness for LimSup automata, namely that a LimSup automaton is GFG if and only if Eve wins the $2$-token game on it.

One direction is direct: if an automaton is GFG, then Eve can use the letter-game strategy to win in $G_2(\A)$, ignoring Adam's moves. The other direction requires more work. We use an additional notion, that of $k$-GFGness, also known as the width of an automaton~\cite{KM19}, which generalises GFGness, in the sense that Eve maintains $k$ runs, rather than only one, and needs at least one of them to be optimal. We will then show that if Eve wins $G_2(\A)$, then $\A$ is $k$-GFG for a finite $k$. Finally, we will show that for automata that are $k$-GFG, for any finite $k$, a strategy for Eve in $G_2(\A)$ can be used to obtain a strategy for her in the letter game. The main novelty in the argument is the decomposition of $\A$ with $k$ weights into $k$ B\"uchi automata that are GFG whenever Eve wins $G_2(\A)$. (The converse does not hold, namely the $k$ B\"uchi automata can be GFG even if Eve loses $G_2(\A)$ -- see \todo{Example...}). The GFG strategies for these B\"uchi automata can then be combined to prove the $k$-GFGness of $\A$.

We start with the definition of $k$-GFGness, which is based on the $k$-runs letter game, generalizing the letter game.

\begin{definition}[$k$-runs letter game]\label{def:kGFG}
A configuration of the game on a LimSup automaton $\A=(\Sigma,Q,\iota,\delta,\gamma)$ is a pair $(\sigma, b^k)$ where $b^k\in \delta^k$ is a tuple of transitions and $\sigma\in\Sigma\cup\{\epsilon\}$ is a letter. (We abuse $\epsilon$ to also be an empty letter.)
A play begins in $(\sigma_0,b_{0,1},...,b_{0,k})=(\epsilon,\iota,\dots,\iota)$ and consists of an infinite sequence of configurations $(\sigma_0,b_{0,1},\dots,b_{0,k})(\sigma_1,b_{1,1},\dots,b_{1,k})\ldots$. 
In a configuration $(\sigma_i,b_{i,1},\dots,b_{i,k})$, the game proceeds to the next configuration $(\sigma_{i+1},b_{i+1,1},\dots,b_{i+1,k})$ as follows.  
\begin{itemize}
\item Adam picks a letter $a$ from $\Sigma$, then
\item Eve chooses for each $b_{i,j}$, ending in some state $q_{i,j}$, a successor transition $b_{i+i,j}\in \delta(q_{i,j},a)$.
\end{itemize}
In the limit, a play consists of an infinite word $w$ that is derived from the concatenation of $\sigma_0,\sigma_1,\ldots$, as well as of $k$  infinite sequences $\rho_1=b_{0,1},b_{1,1},\ldots$, $\rho_2=b_{0,2},b_{1,2},\ldots$ of transitions. Eve wins the play if $\max_{j\in \{1\ldots k\}}\Val(\rho_j) = \A(w)$.

When Eve has a winning strategy in the game, we say that $\A$ is $k$-GFG, or that $GFG_k(\A)$ holds.
\end{definition}


\begin{lemma}\label{cl:2TokenKToken}
Given a LimSup automaton $\A$, if Eve wins $G_2(\A)$ then she also wins $G_k(\A)$ for any $k\in \mathbb{N}\setminus\{0\}$.
\end{lemma}

\begin{proof}
This is the generalisation of~\cite[Thm 14]{BK18}, and the proof is identical, except that rather than building a run that is accepting if Adam's tokens are accepting, Eve builds a run that realises at least the maximal value among Adam's runs. Here we summarise Bagnol and Kuperberg's original proof:

First observe that if Eve wins $G_i(\A)$ then she wins with a positional strategy. (See \cref{rem:positionalGk}.)

Let $s_2$ be a positional winning strategy for Eve in $G_2(A)$. We inductively show that Eve has a winning strategy $s_k$ in $G_k$ for each finite $k$. To do so, we assume a positional winning strategy $s_{i-1}$ in $G_{i-1}(\A)$. The strategy $s_k$ moves a virtual token, in response to the first $i-1$ tokens in $G_i(\A)$, along transitions that combine into a run that achieves at least the supremum of the values of Adam's first $i-1$ runs. By playing $s_2$ against this virtual token and the $i^{th}$ token in $G_i(\A)$, Eve is guaranteed to achieve at least the supremum value of Adam's $i$ runs, making this a winning strategy in $G_i(\A)$.

\end{proof}

\begin{lemma}\label{lem:KGFG-G2iffGFG}
Given a LimSup automaton $\A$, if $GFG_k(\A)$ for some $k\in \mathbb{N}$, then $\A$ is GFG if and only if Eve wins $G_2(\A)$.
\end{lemma}

\begin{proof}
One direction is immediate: If $\A$ is GFG, Eve wins $G_2(\A)$ by ignoring Adam's tokens.
For the other direction, the argument is identical to one used in~\cite{BK18}, which we summarise here.
The strategy $\tau$ for Eve in $GFG_k(\A)$ provides a way of playing $k$ tokens that guarantees that one of the $k$ runs formed achieves the maximal value of the word played by Adam. If Eve wins $G_2(\A)$ then by \cref{cl:2TokenKToken} she also wins $G_k(\A)$, with some strategy $s_k$. To win in the letter game, she can then play $s_k$ against Adam's letters and $k$ virtual tokens that she moves according to $\tau$. The strategy $\tau$ guarantees that one of the $k$ runs built by the $k$ virtual tokens achieves $\Val(w)$; then her strategy $s_k$ guarantees that her run also achieves $\Val(w)$.
\end{proof}


Given a LimSup automaton $\A$, with weights $\{1,\dots, v\}$, we define $v-1$ auxiliary B\"uchi automata $\A_2,\dots,\A_{v}$ with acceptance on transitions, where each $\A_x$ is a copy of $\A$ except that in each transition, instead of its weight $i$, it is accepting if $i\geq x$. Each $\A_x$ recognises the set of words $w$ such that $\A(w) \geq x$.

We now use these auxiliary B\"uchi automata to argue that if $G_2(\A)$, then $GFG_k(\A)$.

\begin{lemma}\label{lem:decomposeG2}
Given a LimSup automaton $\A$ with weights $\{1,\dots, v\}$, if $G_2(\A)$ holds, then for all $x\in \{2,\dots, v\}$, it is also the case that $G_2(\A_x)$ holds.
\end{lemma}

\begin{proof}
Since $\A_x$ is identical to $\A$ except for the acceptance condition or value function, Eve can use in $G_2(\A_x)$ her winning strategy in $G_2(\A)$. Then, if one of Adam's runs sees a B\"uchi transition infinitely often, the underlying transition of $\A$ visited infinitely often has weight at least $x$. Then, Eve's strategy guarantees that her run also sees a value at least as large as $x$, corresponding to a B\"uchi transition in $G_2(\A_x)$.
\end{proof}

\begin{lemma}\label{lem:G2Gk}
Given a LimSup automaton $\A$ with weights $\{1,\dots, v\}$, if $G_2(\A)$ holds, $GFG_{v-1}(\A)$ holds.
\end{lemma}

\begin{proof}
From \cref{lem:decomposeG2}, if $G_2(\A)$ holds, then for all $x\in \{2,\dots, v\}$, it is also the case that $G_2(\A_x)$ holds. Since each $A_x$ is a B\"uchi automaton, this implies that for all $x\in \{2,\dots, v\}$, the automaton $A_x$ is GFG~\cite{BK18}, that is, there are winning strategies $s_x$ for Eve in the letter game on each $\A_x$. Now, in the $v-1$-run letter game $GFG_k(\A)$, Eve can use each $s_x$ to move one token. Then, if Adam plays a word $w$ with some value $\Val(w)=i$, this word is accepted by $\A_i$, and therefore the strategy $s_i$ guarantees that the run of the $i^{th}$ token achieves at least the value $i$, corresponding to seeing a B\"uchi state of $\A_i$ infinitely often.
\end{proof}


Finally, we can combine the $G_2$ and $GFG_{v-1}$ strategies in $\A$ to show that $\A$ is GFG. 

\begin{theorem}\label{thm:G2}
	A nondeterministic LimSup automaton $\A$ is GFG if and only if Eve wins $G_2(\A)$.
\end{theorem}
\begin{proof}
If $\A$ is GFG then Eve can use the letter-game strategy to win in $G_2(\A)$, ignoring Adam's moves. 
If Eve wins $G_2(\A)$ then by \cref{lem:G2Gk} she wins $GFG_{v-1}(\A)$, where $v$ is the number of weights in $\A$, and by \cref{lem:KGFG-G2iffGFG} we get that $\A$ is GFG.
\end{proof}

\begin{theorem}\label{cl:LimSupGFGness}
	Given a nondeterministic LimSup automaton $\A$, the GFGness problem of $\A$ can be solved in quasipolynomial time with respect to its size. For automata with a fixed number of weights, it can be solved in polynomial time with respect to the size of $\A$. 
\end{theorem}
\begin{proof}
It directly follows from \cref{thm:G2} and \cref{lem:solveG2}; the first reducing the GFGness problem to solving $G_2$, and the second showing that it can be done in the stated complexity.
\end{proof}


==> leftover.tex <==
-------------------- Definitions ----------------------


The \emph{nondeterminism in $\A$ is compliant with the value letter games} if Eve wins the value letter-game. The nondeterminism in $\A$ is compliant with the $t$-threshold letter game if Eve wins the $t$-threshold letter-game.
The nondeterminism in $\A$ is compliant with threshold letter games if it is compliant with all $t$-threshold games.



\Subject{History-determinism/Compliance with the letter games}

The letter game defined below is essentially played on the product of a one-player game (belonging to Adam in Eve's leter game and vice-versa) in which the unique player builds an arbitrary $\Sigma$-word $w$ letter by letter while both players choose transitions in $\A$ over the letters of $w$ to build a run over $w$ in $\A$. The winning condition of the game checks whether the run built has either the same value as $w$ or meets a threshold $t$ whenever $w$ does.

\Subject{History-determinism}
An automaton $\A$ is history-deterministic if Eve and Adam have strategies to resolve the nondeterminism and universality, respectively, that guarantee a value at least and at most equal to the value of the word, respectively. 

%A nondeterministic automaton is history-deterministic \cite{Col09} if there is a strategy\footnote{In Section~\ref{sec:Preliminaries}, we formally defined a ``strategy'' with respect to a specific game. Here we abuse the term ``strategy'' to refer to a general total function on finite words.} to resolve the nondeterminism that only depends on the word read so far, i.e., that is uniform for all possible futures. Colcombet generalized this to alternating automata \cite{Col13} by considering such strategies for both players.%, considering a strategy to be a function from a finite sequence of transition conditions and letters to a transition condition, and considering its adequacy in the model-checking game of $\A$ and a word $w$.
%
%
%We first define how to use a strategy $\tau: (\pro{\Sigma}{\BP(Q)})^*\rightarrow \BP(Q)$ for playing in a model-checking game $\game{w}{\A}$, as the history domains are different. Recall that in the model-checking game $\game{w}{\A}$, positions consist of  a suffix of $w$ and a transition condition of $\A$ so histories have type $(\pro{\Sigma^{\omega}}{\BP(Q)})^*$. From such a history $h$, let $h'$ be the history obtained by only keeping the first letter of the $\Sigma^{\omega}$ component of $h$'s elements, that is, the letter at the head of the current suffix. Then, we extend $\tau$ to operate over the $(\pro{\Sigma^{\omega}}{\BP(Q)})^*$ domain, by defining $\tau(h)=\tau(h')$.
%
%For convenience, we often refer to a history in  $(\pro{\Sigma}{\BP(Q)})^*$, as a pair in $\pro{\Sigma^*}{(\BP(Q))^*}$.
%
\begin{definition}[History-determinism] \label{def:HistoryDet}
	
	
	Formally, $\A$ is history-deterministic if there is are two resolvers (translation strategies from ~\cite{Col13}), that is, functions $r_A, r_E \colon \Delta^* \times \BP(Q) \rightarrow \BP(Q)$
	that induce strategies $s_A$ and $s_E$ for Adam and Eve respectively in the value-game $\A\times w$, such that for all plays $\pi$ that agree with $s_A$, $\Val(\pi)\leq A(w)$ and for all plays $\pi$ that agree with $s_E$, $\Val(\pi)\geq A(w)$.
	
	Similarly, $\A$ is $t$-threshold history-deterministic if there are resolvers for both Adam and Eve as above such that in the $t$-threshold game over $\A \times w$, Eve's resolver induces a strategy that guarantees a play $\pi$ with $\Val(\pi)\geq t$ and Adam's resolver induces a strategy that guarantees that $\Val(\pi)<t$.
	
	\todo{Check the type and whether it is clear how it induces a strategy in the value game?}
	
	\kar{To discuss: given that this is just a different way of defining strategies in the letter games, do we want to spell it out just to then prove that it's indeed the same thing?}
	
	
	%\begin{itemize}
	%\item The \emph{nondeterminism in $\A$ is history-deterministic} if there is a strategy $\tau_E: (\pro{\Sigma}{\BP(Q)})^*\rightarrow \BP(Q)$ such that for all $w\in L(\A)$, $\tau_E$ is a winning strategy for Eve in $\game{w}{\A}$.  
	%\item The \emph{universality in $\A$ is history-deterministic} if there is a strategy $\tau_A: (\pro{\Sigma}{\BP(Q)})^*\rightarrow \BP(Q)$ such that for all $w\notin L(\A)$, $\tau_A$ is a winning strategy for Adam in $\game{w}{\A}$.
	%\item $\A$ is \emph{history-deterministic} if its nondeterminism and universality are history-deterministic.
	%\end{itemize}
\end{definition}
%


\Subject{Good for automata composition}

\begin{definition}[Good for automata composition]\label{def:GFAutomataComposition}
	An automaton $\A$ realizing a function $f:\Sigma^\infty \to \Reals$ is \emph{good for automata composition} if for every alternating word (or tree) automaton $\B$ over an alphabet $\Sigma'$ and with $\Sigma$-labeled states, such that the value of a path $\pi$ in its run is $f(\pi)$, the composed automaton $\pro{\B}{\A}$ is equivalent to $\B$.
\end{definition}


\Subject{Good for trees}
\todo{Any ideas on how to extend it to the quantitative setting?}

In the Boolean setting:

The next definition comes from the work in \cite{KSV06,BKKS13} on the power of nondeterminism in tree automata. It states that a nondeterministic word automaton $\A$ is good-for-trees if we can ``universally expand'' it to run on trees and accept the ``universally derived language'' $\UniDerived{L(\A)}$---trees all of whose branches are in the word language of $\A$. 

Observe that every universal word automaton for a language $L$ is trivially good for $\UniDerived{L}$. Therefore,
for universal automata, we suggest that a dual definition is more interesting: its ``existential expansion to trees'' accepts $\ExiDerived{L}$---trees in which there exists a path in $L$. 

For an alternating automaton $\A$, we generalize the good-for-trees notion to require that $\A$ is good for both $\UniDerived{L(\A)}$ and $\ExiDerived{L(\A)}$, when expanded universally and existentially, respectively.

We first formally generalize the definition of ``expansion to trees'' to alternating automata. 
%It follows the standard definition of a run of an alternating automaton on a word, while rather than considering in each step the next letter, it considers the label of a single child or all children of the current tree node: 
The \emph{universal (resp.\ existential) expansion} of $\A$ to trees is syntactically identical to $\A$, while its semantics is to accept a tree $t$ if and only if Eve wins the game $t \times \A$, when $t$ is viewed as a game in which all nodes belong to Adam (resp.\ Eve).


\begin{definition}[Good for trees]\label{def:GFTrees}
	$\A$ is \emph{good for trees} if its universal- and existential-expansions to trees recognize the tree languages $\UniDerived{L(A)}$ and $\ExiDerived{L(A)}$, respectively.
\end{definition}


--------------------- Notion Comparison -----------------------------
\udi{\cref{cl:HDimpliesGFG} seems to be redundant, as it follows from \cref{cl:THDimpliesTGFG,cl:GFGiffTGFG,cl:THDnotHD}}

\udi{History Determinism \Implication Good for Games}
\begin{lemma}\label{cl:HDimpliesGFG}
	If $\A$ is compliant with the value letter game, then $\A$ is good for composition with value games.
\end{lemma}
\begin{proof}
	Assume that the nondeterminism in $\A$ is compliant with the letter-games. Let $s$ be a winning strategy for Eve in her letter-game. We show that for all $\Val$-games $G$, the value $\Val(G)\leq \Val(G\times \A)$.
	Let $s'$ be Eve's strategy in $G$ such that $\Val(\pi)\geq \Val(G)$ for all $\pi$ that agree with $s'$. The choices of Eve in $G\times \A$ consist of the choices of direction at $V_E$ positions in $G$, namely positions $(v,q)\in V_E\times Q$, and disjunctive choices from $\A$, namely positions $(v,b\vee b')\in V\times \BP(Q)$. 
	Let $\hat s$ be the strategy that combined $s$ and $s'$ into a strategy in $G\times \A$ by resolving the choices of direction in $G$ using $s'$ and the disjunctions in $\A$ using $s$. Recall that a play $\pi$ in $G\times \A$ consists of a path $p$ in $G$ and a run $\rho$ of $\A$ over the label $w$ of $p$; The value of $\pi$ is $\Val(\rho)$. Then  using $s'$ to resolve the directions in $G$ guarantees that $\A(w)\geq \Val(G)$ while using $s$ to resolve the nondeterminism in $\A$ guarantees that $\Val(\rho)\geq \A(w)$. We conclude that $\hat s$ guarantees a payoff of at least $\Val(G)$ in $G\times A$. By a symmetric argument, if the universality in $\A$ is compliant with Adam's letter game, then Adam has a strategy to guarantee a payoff at most $\Val(G)$. $G$ and $G\times \A$ are therefore equivalent.
	
	
\end{proof}

\udi{For $\Val$-automata on which the letter-game is determined:\\Threshold History Determinism \DualImplication Threshold Good for Games}
\begin{corollary}
	If the threshold letter game is determined for all automata with some value function $\Val$, then an automaton is good for composition with games if and only if it is compliant with threshold letter games.
\end{corollary}

------------------------------------------------------------------------------------------------------------------------------------

\section{LimInf and LimSup Automata}
B\"uchi and coB\"uchi automata are special cases of LimSup and LimInf automata, by taking the transition weights to be from $0$ and $1$. Therefore, nondeterministic LimSup and LimInf automata cannot be determinized by pruning \cite{BKKS13}, and determinizing nondeterministic LimInf automata involves, in the worst case, at least an exponential size blow-up \cite{KS15}.

Also analogously to B\"uchi and coB\"uchi automata, while nondeterministic LimInf automata can always be determinized, LimSup automata cannot \cite{CDH10}. (Determinizing a nondeterministic LimInf automaton with $n$ states and $k$ different transition weights involves up tp $2^{kn}$ size blow-up \cite{CDH10}.\todo{Give a more exact blowup for $k$ subsets of $Q$, each a subset of the previous one.}) Nevertheless, we show below that a GFG nondeterministic LimSup automata with $n$ states and $k$ different transition weights can always be determinized into a LimSup automaton with at most $n^{2k}$ states.

------------------------------------------------------------------------------------------------------------------------------------


\CheckRelevance{
	\section{Automata on Finite Words}\label{sec:FiniteWords}
	GFG NFAs are known to be determinizable by pruning (DBP) \cite{}. That is, they can be turned into deterministic automata by removing some of their states and transitions. The underlying reason is that in such a GFG automaton, when there are transitions from a state $q$ over a letter $a$ to some states $q_1, \ldots, q_n$, and there is a GFG strategy that chooses at some point the transition $\trans{q}{a}{q_1}$, we must have that $L(\A^{q_1}) \supseteq \cup_{i=2}^{n} L(A^{q_i})$.
	
	Looking into the DBP property with respect to GFG $\Val$-automata on finite words, one should first characterize the value function $\Val$. Observe that a GFG strategy that chooses at some point the transition $\trans{q}{a}{q_1}$ might choose at a different point the transition $\trans{q}{a}{q_2}$, so keeping only  $\trans{q}{a}{q_1}$ might be problematic. It turns out that the crux for the DBP property of GFG NFAs is that their value function, which is to end the run in an accepting state, is ``prefix monotonic''. That is, if the value of the function on one possible suffix of the run is higher than its value on another suffix, then this is also the case when concatenating the suffices to any prefix.
	
	We formalize below the ``prefix monotonic'' property and show that a class of $\Val$-automata on finite words is DBP if and only if $\Val$ is prefix monotonic.
	\begin{definition}
		A value function $\Val$ is \emph{prefix monotonic} if for every finite set $S\subset \Rat$, sequence $\alpha\in S^*$ and sequences $\beta,\beta'\in S^\infty$, if $\Val(\beta)\geq\Val(\beta')$ then $\Val(\alpha\beta)\geq\Val(\alpha\beta')$.
	\end{definition} 
	Observe that the above definition does not consider arbitrary sequences of rational numbers, but rather sequences of finitely-many different rational numbers, which is the case in sequences of weights that are generated by runs of quantitative automata.
	
	
	\begin{theorem}
		A class of $\Val$-automata on finite words is DBP if and only if $\Val$ is prefix monotonic.
	\end{theorem}
	\begin{proof}
		\todo{...}
	\end{proof}
	
	\begin{corollary}
		\todo{For the standard quantitative automata Sup, Inf, Sum, Avg, ... on finite words, GFG automata are DBP.}
	\end{corollary}
	
	\todo{Examples of automata classes that do not have this property. Cost-automata (B,S) that do not have it and indeed in which GFG automata are more expressive than deterministic ones, the simple ``visit red and blue'' automata which do not have and in which GFG automata can be determinized but not by pruning.}
	
	\todo{Speak somewhere on the flexibility of the value function - with no restriction a $\Val$-automaton can model a PDA or a Turing machine.}
	
	\todo{Possibly prove that a $Val$-automaton has the ``children property'' over both finite and infinite words iff $Val$ is prefix monotonic, and from there prove the DBP property of finite words. Doing that, we can also use the children property for infinite words.}
	
} %CheckRelevance

------------------------------------------------------------------------------------------------------------------------------------

\CheckRelevance{
	\todo{K: This probably needs reorganisation as it has nothing to do with one-token games}
	
	\begin{lemma}
		If all GFG-automata $\A$ with value function $\Val$ are DBP, then $\Val$ is prefix monotonic.
	\end{lemma}
	\begin{proof}
		We prove the contrapositive. Assume that $\Val$ is not prefix monotonic: for some finite set $S\subset \Rat$, and sequences $\alpha\in S^*, \beta, beta'\in S^\infty$, we have $\Val(\beta)\> \Val(\beta')$ but $\Val(\alpha\beta)<\Val(\alpha\beta')$.
		
		We can then build an automaton that is not DBP. It has an initial state $\iota$, with an $\alpha$-weighted loop over some word $v_\alpha$. Over a letter $a$ that does not appear in $v_\alpha$, there is a nondeterministic choice to go to one of two deterministic automata $\A$ and $\A'$, with only $\beta$- and $\beta'$-weighted runs respectively. \udi{Such deterministic automata are possible when $\beta$- and $\beta'$ are finite or eventually periodic, but not in general.}
		
		This automaton is GFG: after reading $a$ at the initial state, the future of the word does not affect the value of the word. However, it is not DBP as the maximal value of words starting with $a$ is achieved via the transition to $\A$, while the maximal value of words starting with $v_{\alpha}a$ is achieved via the transition to $\A'$.
	\end{proof}
	
	\todo{
		Showing that if GFG = DBP then the value function is residual seems a lot harder.
	}
} %\CheckRelevance


------------------------------------------------------------------------------------------------------------------------------------



------------------------------------------------------------------------------------------------------------------------------------



------------------------------------------------------------------------------------------------------------------------------------



==> leftoversfrom-intro.tex <==

\NotNeeded{ Then, there are several reasons the synthesis problem might not have a solution:
\begin{itemize}
\item The specification might require the system to predict the future. For example, specifications that require each output to match the next input is not realisable.
\item The projection of the specification on the input component might not be $\Sigma_I^\omega$.
\item The solution might not be computable within the expected transducer model. If there are no restrictions on $L$, then there might be a solution function to the synthesis problem, but it could require infinite memory, or might even be uncomputable.
\end{itemize}
}
 

 %The synthesis problem requires the transducer to guarantee the specification $L$ regardless of the input sequence that describes the environment's behaviour. This means that if it is possible for the environment to misbehave, that is, to produce a sequence of inputs $I\in \Sigma^\omega$ such that no output $O\in \Sigma^\omega$ leads to a global behaviour $I\otimes O\in L$, then the answer to the synthesis problem is "no" and no transducer is generated. However, this can be unrealistic as typically we expect systems to behave correctly \textit{as far as possible}, even if circumstances outside of the control of the system could prevent it from satisfying the specification. For example, we would expect an autonomous vehicle to leave the carpark to attempt to reach its destination even if, theoretically, a road could be blocked, making the destination unreachable in some possible environments. To capture this more permissive variant of the synthesis problem, ``good-enough synthesis'' \cite{AK20} or partial domain synthesis~\cite{} requires that  $I\otimes O\in L$ only if there exists some sequence $O'$, such that $I\otimes O'\in L$.
 
%n recent years there has been a growing interest in quantitative verification and formal methods, in which we not only want a system to satisfy a specification, but we also want it to satisfy it in an optimal way, or while satisfying some quantitative boundary conditions such as energy usage and battery life. A specification is then not a language but a function $f$ from $(\Sigma_I \cdot \Sigma_O)^\omega$ to $\Reals$, and the synthesis problem is generalized from the Boolean setting in several ways \cite{AK20,FLW20}, each requiring the solution function to produce an output sequence $O\in\Sigma_O^\omega$, letter by letter, corresponding to every input sequence $I\in\Sigma_I^\omega$:
%\begin{itemize}
%	\item \emph{Value synthesis} asks for the maximal value $v$ such that the value $f(I\otimes O)$ of all global behaviours  produced by the interaction of the system and the environment is at least $v$ (and the solution guaranteeing $v$).
%	\item \emph{Threshold synthesis}, which generalizes `standard' synthesis, with a given threshold $t\in\Reals$ requires that $f(I\otimes O) \geq t$. (The nonstrict $\geq$ may be replaced with a strict $>$.)
%	\item \emph{Best-value synthesis}, which generalizes the Boolean good-enough synthesis, requires that 
%	$f(I\otimes O) = \sup \{f(I\otimes O') \St O'\in\Sigma_O^\omega\}$. %in case that the supremum is attainable, namely in case that there exists  $O''\in\Sigma_O^\omega$, such that $f(I\otimes O'') = \sup \{f(I\otimes O') \St O'\in\Sigma_O^\omega\}$. \footnote{In \cite{FLW20}, considering synthesis with respect to finite words, a supremum is always attainable, since for every finite input sequence there are finitely may possible output sequences. However, with infinite words this is not necessarily the case. For example, a specification function $f$ over $\Sigma_I=\{a\}$ and $\Sigma_O=\{x,y\}$ that values $I\otimes O$ with $0$ if $O$ has infinitely many occurrences of $x$ and $1-1/(\text{number of $x$'s in $O$})$ otherwise, attains no supremum.}
%	\item \emph{Good-enough threshold synthesis}, which combines threshold synthesis and the Boolean good-enough synthesis, is given a threshold $t$ and requires that $f(I\otimes O) \geq t$ in case that exists some output sequence $O'$ such that $f(I\otimes O') \geq t$. (The nonstrict $\geq$ may be replaced with a strict $>$.)
%	\item \emph{Approximated best-value synthesis} is given a distance metric $d$ and an approximation factor $\alpha>0$ and requires that 
%		$d(f(I\otimes O), \sup \{f(I\otimes O') \St O'\in\Sigma_O^\omega\})\leq \alpha$. (The nonstrict $\leq$ may be replaced with a strict $<$.)
%\end{itemize}

\NotNeeded{
Analogously to the Boolean setting, GFG and history deterministic quantitative automata are closely related to the above quantitative synthesis problems.
We group the above synthesis problems into two groups: on one hand value and threshold synthesis, and on the other best-value, good enough and approximative best-value synthesis. Each category of problems relates to GFGness and history determinism in a different way, as summarised below.

{\bf Value and threshold synthesis:} The value and threshold synthesis problems reduce to solving a quantitative game. Then, the input automaton can be alternating GFG rather than deterministic, without affecting the complexity of realisability. For GFG nondeterministic automata, strategies in the quantitative game are also solutions to the synthesis problem. For alternating GFG automata, while realisability can be solved without additional complexity, the strategy in the quantitative game does not give a solution to the synthesis problem. However, if the input alternating automaton is not just GFG, but also history-deterministic, at least on the universal side, then the witness of the history-determinism of the universality can be combined with the strategy in the quantitative game to produce a solution to the synthesis porblem. Then, the complexity of the witness of history determinism \emph{on the universal side} is crucial for the analysis of the complexity of solutions to the synthesis problem.

{\bf Best-value, good enough and approximative synthesis:} The best-value, good enough $t$-threshold, and approximative best-value realisability problems for deterministic $\Val$-automata (and history-deterministic automata) are logspace equivalent to deciding whether a nondeterministic $\Val$-automaton is history-deterministic, $t$-threshold-history deterministic and approximatively history deterministic, respectively. The witness of history-determinism also induces the solution function, so the versions of these synthesis problems that ask for a solution implementable by a specific model reduces to deciding whether the history-determinism of an automaton has a simple-enough witness.  Similarly, if the input automaton is alternating, but with history-deterministic nondeterminism, then the above realisability problems reduce to deciding whether the nondeterminism in an alternating automaton is ($t$-threshold, approximatively) history-deterministic. \todo{check what the solution depends on}.


The above relationships between synthesis problems and history-determinism motivate further study into both the question of deciding the level of history-determinism of quantitative automata and the question of the complexity of history-determinism witnesses. Inspired by tools to decide the GFGness of B\"uchi and coB\"uchi automata, we address these questions for nondetermistic LimSup automata and show that history-determinism, and therefore best-value synthesis for deterministic (and nondeterministic history-deterministic) LimSUp automata, is solvable in quasipolynomial time, or polynomial time when the number of weights is fixed. However, we also observe that the complexity of the decision problem and of the witness are not necessarily the same, and as a result the realisability problem can be much simpler than exhibiting the witness function.

This final contribution exhibits how tools developed to understand history-determinism can successfully be applied to quantitative synthesis questions, and opens up an exciting direction for addressing the synthesis of various quantitative automata.


%For solving the value synthesis one can express the specification function $f$ by a GFG (instead of deterministic) automaton $\A$ with some value function $\Val$, and then turn $\A$ into a two-player $\Val$ game, allowing Adam to control the input letters and universal choices, and Eve to respond with the output letters and nondeterministic choices. The value of the game is also the value of the synthesis problem for $\A$. Furthermore

%the solution to the synthesis problem is an optimal strategy for Eve.  in case that the optimal value of the game is at least $t$, and `no' otherwise. For the

Motivated by threshold synthesis, it is thus important to understand the potential expressiveness and succinctness of GFG $\Val$-automata, with respect to various $\Val$ functions, compared to deterministic ones.

For solving ($\alpha$-approximated) best-value synthesis, or good-enough $t$-threshold synthesis,
one can express the specification function $f$ by a GFG $\Val$-automaton $\A$, and then turn $\A$ into a ``more nondeterministic'' $\Val$-automaton $\A'$, by merging all the output letters to a single letter. The synthesis problem has a solution if and only if $\A'$ is ($\alpha$-)GFG, or $t$-threshold GFG respectively, and a solution is a strategy that witnesses $\A'$'s GFGness.

For best-value synthesis, it is thus also important to understand the decidability and complexity of the GFGness problem of various $\Val$-automata.

\todo{Do we see a nice GFG formulation of the Good-enough threshold synthesis problem?}

\todo{Check for other papers on quantitative synthesis.}
}
%The quantitative synthesis problem can be viewed as a two player game $\G$ between the `environment' and the `system', where the environment chooses the input letters and the system chooses the output letters, and the award function of the game is the specification function $f$. 
%As in the Boolean setting, a deterministic quantitative automaton $\D$ realizing the specification function $f$ can be used in solving the synthesis problem---the product of $\G$ and $\D$ is a game whose award function is the value function of $\D$ and that is equivalent to $\G$. That is, $\G$ and $\G\times\D$ have the same optimal value and an optimal strategy in one game can be directly translated to an optimal strategy in the other.
%Hence, GFG quantitative automata, which are good-for-game-composition, can replace deterministic automata in solving quantitative synthesis.

\NotNeeded{
\Subject{Related work}\

\cite{AKL10}: Considering $\Func{sum}$-automata and approximations with respect to the \textit{ratio} metric, they define a nondeterministic automaton $\A$ to be \emph{$(\alpha,r)$-determinizable by pruning}, for an approximation factor $\alpha \geq 1$ and an integer $r \geq 0$, if the $r$-refinement of $\A$ embodies a deterministic automaton that $\alpha$-approximates $\A$ \cite[Definition 3.1]{AKL10}. An $r$-refinement together with embodiment of an automaton $\A$ is analogous to taking its product with a (memory) transducer of up to $2^r$ states. We thus have that {$(\alpha,r)$-determinization by pruning is equivalent to $\alpha$-GFGness with respect to a fixed memory of size $2^r$ and the \textit{ratio} metric, and that {$(1,0)$-determinization by pruning is equivalent to standard determinization by pruning.

They show that the DBPness problem of nondeterministic $\Func{sum}$-automata can be solved in polynomial time \cite[Theorem 4.2]{AKL10}, 
and that a $\Func{sum}$-automaton is GFG with finite memory iff it is DBP \cite[Theorem 5.1]{AKL10}.
Together with the result that a $\Func{sum}$-automaton is GFG if and only if it is GFG with finite memory \todo{Is there such a result?}, we get that the GFGness problem of nondeterministic $\Func{sum}$-automata can be solved in polynomial time.

\cite{HPR15,HPR17}: Considering two-player (Eve and Adam) zero-sum games, they are interested in strategies of Eve that minimize her regret, i.e.\ strategies that minimize the difference between her actual payoff and the payoff she could have achieved if she had known the strategy of Adam in advance. 
They consider three classes of strategies, one of which is ``word strategies'', under which the considered game is analogous to the ``GFG letter-game'' over a nondeterministic quantitative automaton. 

Given a distance metric $d$ and an approximation factor $\alpha$, they define  \cite[before Proposition 3]{HPR17} a nondeterministic quantitative automaton $\A$ to be
\emph{(strictly) $\alpha$-good for games} if Eve has a strategy in the letter game that guarantees for every word $w$ a value $v$, 
 such that $d(v,\A(w)) \leq \alpha$ (resp.\ $d(v,\A(w)) < \alpha$).
  
They look into $\alpha$-GFGness of quantitative automata over infinite words, considering the \textit{difference} metric and the value functions: $\Func{Inf}, \Func{Sup}, \Func{LimInf}, \Func{LimSup}, \Func{LimInfAvg}$ (called $\underline{MP}$), and $\Func{LimSupAvg}$ (called $\overline{MP}$).

They show that given an approximation factor $\alpha$, deciding if a nondeterministic automaton is $\alpha$-GFG (strictly or non-strictly) with respect to the \textit{difference} metric is EXPTIME-complete for $\Func{Inf}$-, $\Func{Sup}$-, $\Func{LimInf}$-, and $\Func{LimSup}$-automata; and it is undecidable for 
$\Func{LimInfAvg}$- and $\Func{LimSupAvg}$-automata \cite[Theorem 3]{HPR17}. Considering a fixed memory bound for the GFG strategy, they show that the GFGness problem is NP-complete with respect to the automaton size and the memory bound for nondeterministic automata of all the six value functions above. (Notice that $\Func{Inf}$-, $\Func{Sup}$-, $\Func{LimInf}$-, and $\Func{LimSup}$-automata are GFG if and only if they are GFG with a memory exponentially bounded in the size of the automaton, while this is not the case for  $\Func{LimInfAvg}$- and $\Func{LimSupAvg}$-automata \cite[Corollary 3]{HPR17}.)

\todo{Does their undecidability result hold even if the approximation ratio is $0$?}


\cite{HPR16}: The authors of \cite{HPR15,HPR17} continue their research, handling $\Func{discounted}$-$\Func{sum}$-automata on infinite words. In this paper they also consider the \emph{regret-free} problem, namely the $0$-GFGness (standard GFGness) problem, which turns out to be simpler -- NP-complete \cite[Theorem 6]{HPR16}, as opposed to $\alpha$-GFGness, for which the paper does not give a general solution, while giving an EXPTIME solution for the case that the discount factor is $\lambda=\frac{1}{n}$, for an integer $n>1$  \cite[Theorem 7]{HPR16}, and a PSPACE-complete ``approximated solution'' for the general case \cite[Theorems 8,9]{HPR16}. In \cite[proof of Theorem 6]{HPR16}, they also show that a $\Func{discounted}$-$\Func{sum}$-automaton is GFG if and only if it is DBP.

\cite{FJLPR17} continues the work of \cite{AKL10}, though with respect to the \textit{difference} metric rather than the \textit{ratio} metric, and in particular shows that deciding if exists for a given $\Func{sum}$-automaton $\A$ an approximation factor $\alpha$ such that $\A$ is $\alpha$-DBP is EXPTIME-complete \cite[Theorems 7 and 8]{FJLPR17}.

\cite{FLW20}


Thomas Colcombet’s original definition of `history determinism' \cite{Col09} already relates to non-Boolean automata, considering cost automata. While the restriction of his definition to $\omega$-regular automata coincides with the original definition in \cite{HP06} of good for games automata \cite{BL19}, in the quantitative setting his definition is quite different from what we provide here.
In comparison to our definition, his notion can be viewed as `approximated history-deterministic with respect to a threshold': an automaton $\A$ satisfies Colcombet’s definition if there is an approximation ratio $\alpha$, such that for every threshold $n$, there is a strategy $\delta_n$ that the automaton can follow and achieve a value up to $\alpha$ worse than the value that full nondeterminism provides, with respect to words whose value with full nondeterminism is below the threshold $n$. 

}

==> onetoken.tex <==

Bagnol and Kuperberg showed that $G_1$, the one-token version of $G_2$ does not suffice to characterise GFGness for B\"uchi automata~\cite[Lemma 8]{BK18}. However, $G_1$ turns out to be sufficient for checking whether some quantitative automata are GFG.


On finite words, $G_1$ is defined as earlier, except that the winning condition is a safety condition for Eve: for all finite prefixes of a play, it must be the case that the value of Eve's run is at least the value of Adam's run.


\begin{theorem}\label{cl:G1residual}
Given a nondeterministic automaton $\A$ with a \residual value function $\Val$ over finite or infinite words,
Eve wins $G_1(\A)$ if and only if $\A$ is GFG.
\end{theorem}

\begin{proof}
One direction is immediate: if $\A$ is GFG then Eve can use her GFG strategy to win $G_1$ by ignoring Adam's token.

For the other direction, assume that Eve wins $G_1$. Now consider the following family of \textit{copycat strategies} for Adam in $G_1$: a copycat strategy is one where Adam moves his token in the same way as Eve until she makes a non-residual move $q\xrightarrow{a}q'$ after building a run $\rho$. If Eve makes a non-residual move, then the copycat strategies stop copying Eve and direct Adam's token along the run $\pi'$ over $aw$ from $q$ that maximises $\Val(\rho \pi')$ and plays the word $w$. Observe that if Eve is playing in $G_1$ against a copycat strategy and plays a non-residual move, then she loses.

If Eve wins $G_1$ with a strategy $s$, then she wins in particular against all copycat strategies and therefore $s$ never makes a non-residual move against such a strategy.

Eve can then play in the letter game over $\A$ with a strategy $s'$ that moves her token as $s$ would in $G_1(\A)$ assuming Adam uses a copycat strategy. Then, $s'$ guarantees that she never makes a non-residual move and is therefore a residual strategy. Since $\Val$ is residual, any residual strategy, and in particular $s'$, is winning in the letter game, so $\A$ is GFG.

\end{proof}

\paragraph*{Solving token games}
For resolving the GFGness problem of residual quantitative automata, it then remains to study for which of them the corresponding $G_1$ game is easy to decide.

\begin{corollary}\label{cl:Ptime}
Deciding whether an Inf-automaton or Sup-automaton on finite words is GFG is in PTime.
\todo{We can possibly also detail the exact upper bounds that we have for each automaton type.}
\end{corollary}

\begin{proof}
Given a Sup automaton $\A=(\Sigma,Q,\iota,\delta,\gamma)$ with weights $W$,  $G_1(\A)$ reduces to solving a safety game, whose positions $(\sigma,q,q',x_E, t)\in \Sigma\cup\varepsilon\times Q^2\times W\times \{l,e,a\}$ consist of a possibly empty letter $\sigma$ representing the last letter played, a pair of states $(q,q')$, one for Eve and one for Adam, which keep track of the end of the current run built by each player, weight $x_E$ from $W$, which keeps track of the maximal weight seen on Eve's run so far, and a turn variable $t\in \{l,e,a\}$ indicating whether it is Adam's turn to give a letter ($l$), Eve's turn to choose a transition ($e$), or Adam's turn to choose a transition ($a$). The initial position is $(\iota,\iota,m,m)$ where $m$ is the minimal weight of $\A$.
Similarly to the construction in the proof of~\cref{lem:solveG2}, the moves and position ownership encode the permitted moves in $G_1(\A)$ and update $x_E$ to reflect the maximal value of Eve's run.

The winning condition for Eve is a safety condition: Adam wins if he picks a move with a weight higher than $x_E$, the maximal weight on Eve's run. Then plays in this game are in bijection with plays of $G_1(\A)$, and Eve wins if and only if she can avoid Adam choosing a transition with a larger weight than $x_E$, that is, if she can win $G_1(\A)$. 

Then, solving $G_1(\A)$ reduces to solving this safety game, which is of size $3n^2p$, where $n$ is the size of $\A$ and $p$ is the number of weights. \todo{As safety games can be solved in time ... \cite{...}, we get that checking the GFGness of sup automata is in $O(...)$.}

The case of Inf-automata is similar, except that $x_E$ keep track of the minimal value of Eve's run, starting with the maximal weight of $\A$, and the safety condition for Eve is that $x_E$ must be smaller than any weight picked by Adam.

The case of Inf-automata is similar, except that $x_E$ and $x_A$ keep track of the minimal value of both players' runs, starting with the maximal weight of $\A$, and the safety condition for Eve is that $x_E\leq x_A$.
\end{proof}


\CheckRelevance{
\begin{corollary}\label{cl:Ptime}
	Deciding whether Sum- or Avg-automaton on finite words is GFG is in PTime.
\end{corollary}
\begin{proof}
\paragraph*{Sum}
Given a Sum automaton $\A=(\Sigma,Q,\iota,\delta,\gamma)$ with weights $W$, the game $G_1(\A)$ can also be reduces to a sum game: similarly to the proof of~\cref{lem:solveG2}, 
\udi{Why do we refer to \cref{lem:solveG2} and not to the previous part of this proof, which speaks of Sup automata? The positions look the same.}
	the positions and moves of $G_1(\A)$ can be encoded into a game with positions in $\Sigma\cup\varepsilon\times Q^2\times\{l,e,a\}$ (since Adam has only one run, only two states of $Q$ are needed), so that its plays are in bijection with those of $G_1(\A)$. 

 To encode the winning condition, each move corresponding to a choice of transition by Eve is endowed with the weight of the chosen transition, and moves corresponding to Adam's choices of transitions are endowed with the negation of the weight of the chosen transition. Other moves have weight $0$. This ensures that at the end of any play prefix ending in an $l$ position, the sum of the weights on the play is the difference between the sum of the weights on Eve's and Adam's runs in $G_1(\A)$. We also add a sink position to which Adam can move from any $l$-position and where there is only a $0$-weighted self-loop. This lets Adam choose to end the game at any turn.

Then, if Eve wins $G_1(\A)$, she can ensure that the sum of the weights so far in the constructed game is non-negative at all $l$-positions. Conversely, if Adam wins $G_1(\A)$, then he can ensure that this sum is negative at some $l$-position, from where he can move to the neutral sink.

This is nearly a $0$-threshold Sum game, 
\udi{The game setting fits the ``fixed initial credit problem'' of ``energy games'', known to be equivalent to mean-payoff games, and is therefore in $NP \cap coNP$, currently only having an exponential deterministic algorithm.}
except that the sum might dip briefly under $0$ between Eve and Adam's choices of transition. This is easy to fix by using a single weight, the difference of the weights between Eve and Adam's transition into a single weight. This adds a factor of $W$ to the size of the game.

Then, solving $G_1(\A)$ reduces to solving a $0$-threshold Sum game of polynomial size in $\A$. \todo{Give the exact upper bound that we get.}

\kar{Is this clear or should we describe this game directly?}.
\udi{I think that it may be better to directly give the latter game, as we also use a variant of it in the discounted-sum case.}

\todo{What's the reference for solving these games?}

\paragraph*{Avr}
\udi{Isn't the average case exactly like the sum case? Since the runs of Eve and Adam are of the same length, a run of Adam has a higher average iff it has a higher sum.}
The case for Avr-automata reduces to an Avr-game with a similar construction as above, in which the weights on Adam's run are negated. And the sinks are target states. Then the average of the weights on a play ending in a target state is the average difference between the weights on Eve's run and the weights in Adam's run. This in turn is the difference between the average of weights on Eve's run and the average of weights on Adam's run.

\kar{Do we know how to solve such games in P?}

\end{proof}
} %\CheckRelevance

\begin{corollary}\label{cor:DSum-NPcoNP}
Deciding whether a DSum automaton $\A$, on finite or infinite words, is GFG is {\sc NP}$\cap${\sc co-NP}\footnote{This is perhaps surprising, given the NP-hardness result in~\cite[Theorem 6]{HPR16}. In consultation with the authors, we have confirmed that there is an error in the hardness proof.}. 
\end{corollary}

\begin{proof}
Consider a $\lambda$-DSum automaton $\A=(\Sigma,Q,\iota,\delta,\gamma)$.
From~\cref{cl:finite-is-present-oriented,lem:DSum-present-oriented,cl:G1residual}, Eve wins $G_1(\A)$ if and only if $\A$ is GFG. It therefore suffices to show that solving $G_1(\A)$ is {\sc NP}$\cap${\sc co-NP}. We achieve this by reducing solving $G_1(\A)$ to solving a discounted-sum game. It is enough to consider infinite games, as they also encode finite games, by allowing Adam to move to a forever-zero-position in each of his turns.

The reduction follows the same pattern as those in the proof of \cref{cl:Ptime}: we represent the arena of the game $G_1(\A)$ as a finite arena, and encode its winning condition, which requires the difference between the DSum of two runs to be non-negative, as a threshold DSum winning condition. The key to doing this is observing that the difference between the $\lambda$-DSum of the two sequences $v_0v_1...$ and $v'_0v'_1...$ of weights is equal to the $\lambda$-DSum of the sequence of differences $d_0=(v_0-v'_0), d_1=(v_1-v'_1), \ldots$, as follows:

\[
(\sum_{i=0}^\infty \lambda^i v_i ) - \sum_{i=0}^\infty \lambda^i v'_i  = \sum_{i=0}^\infty \lambda^i (v_i-v'_i) 
\]

We now describe the DSum arena $G$ in which Eve wins with a non-strict $0$-threshold objective if and only if she wins $G_1(\A)$.
The arena has positions in $(\sigma,q,q',d,t)\in \Sigma\cup \varepsilon \times Q^2 \times \delta\cup \varepsilon \times \{l,e,a\}$ where $\sigma$ is the potentially empty last played letter, starting with $\varepsilon$, the states $q,q'$ represent the positions of Eve and Adam's tokens, $d$ is the transition just played by eve if $t=a$ and $\varepsilon$ otherwise. Moves between positions capture the permitted moves in $G_1(\A)$.

Adam's  moves that choose transitions, namely $(\sigma,q,q',d,a)\rightarrow(\sigma,q,q'',\varepsilon,l)$, are given weight $\gamma(d)-\gamma(q',\sigma,q'')$, that is, the difference between the weights of the transitions chosen by both players.

Other transitions are given weight $0$. To compensate for the fact that only one edge in three is weighted, the discount factor $\lambda'$ of the DSum game $G$ is set to $\lambda^{\frac{1}{3}}$.

Then plays in $G_1(\A)$ and in $G$ are in bijection. It now suffices to argue that the winning condition of $G$, namely that the $\lambda^{\frac{1}{3}}$-DSum of the play is non-negative, correctly encodes the winning condition of $G_1(\A)$, namely that the difference between the $\lambda$-DSum of Eve's run and of Adam's run is non-negative.

We now argue that the $\lambda^{\frac{1}{3}}$-DSum of a play of this game is non-negative if and only if the $\lambda$-DSum of the sequence of weight differences $d_0 d_1 \ldots$ between the transitions played by both players is non-negative. Indeed, the $\lambda^{\frac{1}{3}}$-DSum is equal to the required DSum multiplied by $\lambda^{\frac{2}{3}}$ -- each play of the $\lambda^{\frac{1}{3}}$-DSum encounters two $0$-weights, then the weight $d_i$ at the $(3i)^{th}$ move, so:

\[
\lambda^{\frac{1}{3}}\text{-DSum} = 
\sum_{i=0}^\infty (\lambda^{\frac{1}{3}})^{3i} \cdot  d_i  ~+  (\lambda^{\frac{1}{3}})^{3i-1} \cdot 0 + (\lambda^{\frac{1}{3}})^{3i-2} \cdot 0 
= \lambda ^{-\frac{1}{3}}\sum_{i=1}^\infty \lambda^i d_i 
= \lambda^{\frac{2}{3}} \sum_{i=0}^\infty \lambda^i d_i 
\]

Hence Eve wins the game $G_1(\A)$ if and only if she wins the $0$-threshold $\lambda^{\frac{1}{3}}$-DSum game over $G$.
As $G$ is of size polynomial in the size of $\A$ and solving DSum-games is in {\sc NP}$\cap${\sc coNP}~\cite{ZP95}, solving $G_1(\A)$, and therefore deciding whether $\A$ is GFG, is also in {\sc NP}$\cap${\sc coNP}. 

\end{proof}

\begin{corollary}
	GFGness check of $\Sum$ and $\Avg$ automata is in PTime.
\end{corollary}
\begin{proof}
	A direct consequence of \cref{cl:SumHdDBP} and \cite[Theorem 4.1]{AKL10}, where the latter shows that DBPness check of $\Sum$ (and $\Avg$) automata is in PTime.
\end{proof}




==> synthesis.tex <==

Establishing the non-equivalence of history-determinism, good-for-gameness and their threshold versions leaves us with the question of which definitions, if any, are the most useful or interesting ones. We explore this question from the perspective of various quantitative synthesis problems and clarify which definitions from Section~\ref{sec:QuantitativeGfgDefinitions} are relevant for each synthesis problem, and how the realisability and synthesis problems relate in each case. We only consider specifications over infinite words, although we expect similar reductions to work for the finite case.

\Subject{Notation} We recall first that a synthesis problem has a specification $f: (\Sigma_I \times \Sigma_O)^\omega \rightarrow \mathbb{R}$ that assigns real values to global behaviours $I\otimes O$. We write $\best{f}{I}$ for $\sup_{O\in\Sigma_O^\omega} f(I\otimes O)$, the best value of a global behaviour involving an input $I$ according to $f$.
The potential solutions to a synthesis problem consist of functions $s:\Sigma_I^* \rightarrow \Sigma_O$ that produce the next output, given a sequence of inputs read so far. Given a finite or infinite sequence $I\in \Sigma_I^*$ or $\Sigma^\omega$, we write $\out{s}(I)$ for the sequence $s(I_0)s(I_1)...$.

\subsection{Best Value Synthesis}

We first consider a version of synthesis interested in how a reactive system can perform in comparison to the maximal value among global behaviours that involve the input.

\begin{description}
\item[Input] Specification $f: (\Sigma_I \times \Sigma_O)^\omega \rightarrow \mathbb{R}$
\item[System] Function $s:\Sigma_I^* \rightarrow \Sigma_O$ such that for all $I\in \Sigma^\omega$ we have $f(I\otimes \out{s}(I))=\best{f}{I}$.
\item[Realisability] Does such a function $s$ [with memory $M$] exist?
\item[Synthesis] If yes, output a transducer with memory $M$ implementing $s$. 
\end{description}

Note that since $\best{\A}{I}$ is a supremum of a set of values, it may not actually be atainable by any word. In this case, the best-value synthesis problem is unrealisable, even if the system could force a value arbitrarily close to $\best{\A}{I}$. Approximative synthesis is a more permissive version of the synthesis problem, which requires the system to guarantee some bound on the distance between the best value and the achieved value.


\begin{description}
\item[Input] Specification $f: (\Sigma_I \times \Sigma_O)^\omega \rightarrow \mathbb{R}$, regret threshold $r\in \mathbb{Q}$ \kar{$\mathbb{Q}? \mathbb{R}?$ More complex distance measure?}
\item[System] Function $s:\Sigma^*_I \rightarrow \Sigma_O$ such that for all $I\in \Sigma_I^\omega$,  $\best{f}{I} - \Val(I\otimes \out{s}(I))\leq r$.
\item[Realisability] Does such a function $s$ [implementably by a computational model $X$] exist?
\item[Synthesis] If yes, output an $X$ implementing $s$.
\end{description}


We now observe that the best value synthesis problem of deterministic (or even GFG nondeterministic) automata and the problem of deciding whether a nondeterministic automaton is history-deterministic reduce to each other.  The relationship between good-enough synthesis~\cite{AK20} and history determinism was already noted for nondeterministic visibly pushdown automata in~\cite{GJLM21}. Furthermore, in~\cite{FLW20} the authors reduce the approximative best value (partial domain) synthesis of deterministic quantitative automata over finite words by finite transducers to the notion of $r$-regret determinisability, which asks whether a nondeterministic automaton can be turned into a deterministic automaton by pruning its product with a finite memory, such that the difference between the value of words in the two automata is bounded by $r$. The results of this section are in exactly the same spirit, although we relate the synthesis problem to history determinism rather than determinisability, and obtain a two-way correspondence for all history deterministic nondeterministic quantitative automata. In the alternating case, only one direction is preserved, and only for reaslisability, rather than synthesis.

   %and in the context of regret-minimisation in~\cite{HPR15}.

\begin{lemma}
Deciding the best value synthesis problem of a history deterministic nondeterministic $\Val$-automaton $\A$ reduces linearly to deciding whether a nondeterministic $\Val$-automaton $\A'$ is history deterministic. Furthermore, the witness of history determinism of $\A'$ is implementable by the same computational models as a solution to the best-value synthesis of $\A$.
\end{lemma}


The idea of the reducton is to turn the output letter choices expected from the solution to the synthesis problem of a deterministic automaton $\A$ into nondeterministic choices in $\A'$. In practice this can be done by taking $\A'$ to be the projection of $\A$ onto the first component of the input letters, making $\A'$ an automaton that maps inputs $I\in \Sigma_I^\omega$ onto $\sup_{O\in \Sigma_O^\omega}\A(I\otimes O)$. Then, a solution to the synthesis problem for $\A$ corresponds exactly to a function that resolves the nondeterminism of $\A'$ on the fly while maximising the value of the run, in other words, a witnesses of the history-determinism of $\A'$. If $\A$ is itself nondeterministic, then $\A'$ will have both the nondeterminism of $\A$ and the nondeterminism that stems from the choice of output letters. As long as the nondeterminism of $\A$ is history deterministic, the nondeterminism of $\A'$ is history deterministic if and only if $\A$ is best value realisable.

\kar{For the appendix:}
\begin{proof}
First let us define formally the projection of $\A$ onto its first component: $\A'=(\Sigma_I,Q,\iota,\delta',\gamma')$, where $\delta(q,a)=\bigvee_{b\in \Sigma_O} \delta(q,(a,b))$.
In other words, the automaton $\A'$ moves the $\Sigma_O$ letters from the input word into a nondeterministic choice. It implements a mapping of inputs $I\in \Sigma_I^\omega$ onto $\best{\A}{I}$. We now argue that witnesses of history-determinism for $\A'$ coincide with solutions to the best-value synthesis problem for $\A$. Let $s$ be the witness of the history-determinism of $\A$.


We first argue that a solution $s'$ to the best-value synthesis problem for $\A$, combined with $s$ is a witness that $\A'$ is history-deterministic. Indeed, in Eve's letter game on $\A'$, Eve has two types of choices: a choice $\bigvee_{b\in \Sigma_O} \delta(q,(a,b))$ of an $\Sigma_O$-letter, and the choice in $\delta(q,(a,b))$ that stems from $\A$. Let $\hat{s}$ be the strategy that after a run prefix $\rho$ ending in a state $q$ over a word $w\in \Sigma_I$ chooses the letter $s'(w)$, that is, the disjunct $\delta(q,(a,s'(w)))$ in the disjunction $\bigvee_{b\in \Sigma_O} \delta(q,(a,b))$. Then, from $\delta(q,(a,s'(w)))$, $\hat{s}$ behaves as $s$ would after a run of $\A$ over $w\otimes\out{s}(w)$.

First, observe that a run $\rho$ of $\A'$ over $I\in \Sigma_I^\omega$, labelled with the choices of $\Sigma_O$-letters forming some $O\in \Sigma_O^\omega$, corresponds to a run of $\A$ over $I\otimes O$ with the same value.

Then, since $s'$ is a solution to the best value synthesis problem, it guarantees that given an input word $\Sigma_I$, the sequence of $\Sigma_O$ letters chosen by $\hat{s}$ is $\out{s}(I)$, and $\A(I\otimes \out{s}(I))=\best{\A}{I}$. Then, as $s$ witnesses the history determinism of $\A$, $\hat{s}$ guarantees that $\rho$ has value $\A(I\otimes \out{s}(I)$, that is, $\hat{s}$ witnesses the history determinism of $\A'$.


For the converse direction, assume $\A'$ is history deterministic, as witnessed by some strategy $s$. We claim that $s$ induces a solution $s'$ to the synthesis problem for $\A$ as follows: after reading an finite sequence of inputs $Ia\in \Sigma_I^*$, $s$ has built some run $\rho$ over $I$ that ends in a state $q$, after which $s$ resolves a disjunction $\bigvee_{b\in \Sigma_O} \delta(q,\binom{a}{b})$ by choosing some $b\in \Sigma_O$. We then set $s'(Ia)=b$. Then, as $s$ witnesses that $\A'$ is history-deterministic, the run chosen by $s$ over an input $I\in \Sigma_I^\omega$ has the value $\best{\A}{I}$. By construction of $\A'$ and $s'$, this is the value  $\A(I\otimes \out{s'}(I)$, that is, $s'$ is indeed a solution to the synthesis problem on $\A$. Furthermore, observe that an implementation of $s$ also implements $s'$ by ignoring the outputs of $s$ that do not choose $\Sigma_O$ letters, so the memory of the solution to the synthesis problem is bounded by the memory required by a witness of history determinism.
\end{proof}


\begin{lemma}
Deciding whether a nondeterministic $\Val$-automaton $\A$ is history-deterministic reduces linearly to deciding the best value synthesis problem of a deterministic $\Val$-automaton $\A'$. Furthermore, the witness of history-determinism of $\A$ is implementable by the same computational models as the solution to the synthesis problem of $\A'$.
\end{lemma}


Dually to the previous translation, we turn the nondeterminism in an automaton $\A$ into choices of output letters in the best-value synthesis problem. Indeed, we can build a deterministic automaton $\A'$ that is similar to $\A$ except that it reads both an input letter and a transition; then a transition can only be chosen if it is the second element of the input (that is, the output letter). Then $\A'$ maps valid runs of $\A$ to their value and a solution to the best value synthesis problem of $\A'$ corresponds exactly to a witness of history-determinism for $\A$.


\begin{proof}
Let $\A'$ be the $\Val$-automaton $(\Sigma \times \Delta, Q,\iota,\delta')$
where $\delta'(q,(a,q\xrightarrow{a:x}q'))= (x,q')$ if $(x,q')\in \delta(q,a)$. $\A'$ maps valid runs of $\A$ written as pairs $(w,r)$ where $r$ is a run of $\A$ over $w$, onto $\Val(r)$ and in particular $\best{\A'}{I}=\A(I)$.

We claim that $\A'$ is best-value realisable if and only $\A$ is history-deterministic. Indeed,  a solution $s$ to the best value synthesis problem of $\A'$ corresponds to a function building a run of $\A$ over the input $I$ transition by transition such that the value of the run is $\best{\A'}{I}$. Since $\best{\A'}{I}$ is $\A(I)$, $s$ is precisely a witness of history-determinism in $\A$. Similarly, a witness of history-determinism in $\A$ induces a solution to the best value synthesis problem for $\A'$ since it builds a run of $\A$ over $I$ with value at least $\A(I)$, exactly what is required from a solution to the best value synthesis.

\end{proof}

We observe that the same proofs extend to the case of alternating automata in which the nondeterminism is history-deterministic: for these automata, the best value synthesis problem of $\A$ corresponds to deciding whether the nondeterminism in an alternating automaton $\A'$ that maps $I$ to $\best{\A}{I}$ is history-deterministic, and, conversely, deciding whether the nondeterminism in an alternating automaton is history-deterministic reduces to solving the best-value synthesis problem for a \textit{universal} automata. In particular, the best value synthesis problem is no easier for universal automata than for alternating automata with history-deterministic nondeterminism.

\begin{lemma}
Deciding the best-value synthesis problem of a history-deterministic alternating $\Val$-automaton $\A$ in reduces linearly  to deciding whether an alternating $\Val$-automaton $\A'$ in which Adam wins his letter-game is history deterministic.
\end{lemma}

Interestingly, the complexity of the solution of the best-value synthesis of $\A$ depends not only on the witness of history-determinism of the nondeterminism of $\A'$, but also on the witness of history determinism of the \textit{universality} of $\A$.
 
\kar{For the appendix:}
\begin{proof}
As before, the projection of $\A$ onto its first component is $\A'=(\Sigma_I,Q,\iota,\delta',\gamma')$, where $\delta(q,a)=\bigvee_{b\in \Sigma_O} \delta(q,(a,b))$. Since $\A$ is history deterministic, the automaton $\A'$ implements a mapping of inputs $I\in \Sigma_I^\omega$ onto $\best{\A}{I}$.
We further observe that the universality of $\A'$ remains history deterministic, using essentially the same witness strategy (excpet that it now reads inputs of $\A'$ rather than of $\A$).


We now argue that witnesses of history-determinism for the nondeterminism of $\A'$ coincide with solutions to the best-value synthesis problem for $\A$. Let $s_E$ and $s_A$ be the witness of the history-determinism of $\A$, and $s'_A$ the witness of the history determinism of the universality of $\A'$.


We first argue that a solution $s'$ to the best-value synthesis problem for $\A$, combined with $s_E$ is a witness that the nondeterminism of $\A'$ is history-deterministic. Indeed, in Eve's letter game on $\A'$, Eve has two types of choices: a choice $\bigvee_{b\in \Sigma_O} \delta(q,(a,b))$ of an $\Sigma_O$-letter, and the choice in $\delta(q,(a,b))$ that stems from $\A$. Let $\hat{s}$ be the strategy that after a run prefix $\rho$ ending in a state $q$ over a word $w\in \Sigma_I$ chooses the letter $s'(w)$, that is, the disjunct $\delta(q,(a,s'(w)))$ in the disjunction $\bigvee_{b\in \Sigma_O} \delta(q,(a,b))$. Then, from $\delta(q,(a,s'(w)))$, $\hat{s}$ behaves as $s_E$ would after a run of $\A$ over $w\otimes\out{s}(w)$.

First, observe that a run $\rho$ of $\A'$ over $I\in \Sigma_I^\omega$, labelled with the choices of $\Sigma_O$-letters forming some $O\in \Sigma_O^\omega$, corresponds to a run of $\A$ over $I\otimes O$ with the same value.

Then, since $s'$ is a solution to the best value synthesis problem, it guarantees that given an input word $\Sigma_I$, the sequence of $\Sigma_O$ letters chosen by $\hat{s}$ is $\out{s}(I)$, and $\A(I\otimes \out{s}(I))=\best{\A}{I}$. Then, as $s_E$ witnesses the history-determinism of $\A$, $\hat{s}$ guarantees that $\rho$ has value $\A(I\otimes \out{s}(I)$, that is, $\hat{s}$ witnesses the history-determinism of $\A'$.


For the converse direction, assume $\A'$ is history-deterministic, as witnessed by some strategy $s$. We claim that $s$, combined with $s'_A$, induces a solution to the synthesis problem and a witness of history-determinism for the nondeterminism of $\A$. Indeed, $s$ and $s'_A$ induce a solution $s'$ to the synthesis problem of $\A$ as follows: after reading an finite sequence of inputs $Ia\in \Sigma_I^*$, $s$ and $s'_A$ have built some run $\rho$ over $I$ that ends in a state $q$, after which $s$ resolves a disjunction $\bigvee_{b\in \Sigma_O} \delta(q,\binom{a}{b})$ by choosing some $b\in \Sigma_O$. We then set $s'(Ia)=b$. Then, as $s$ and $s'_A$ witness that $\A'$ is history-deterministic, the run chosen by $s$ and $s'_A$ over an input $I\in \Sigma_I^\omega$ has the value $\best{\A}{I}$. By construction of $\A'$ and $s'$, this is the value  $\A(I\otimes \out{s'}(I)$, that is, $s'$ is indeed a solution to the synthesis problem on $\A$. The complexity of the implementation of $s'$ depends on both $s$ and $s_A$.
\end{proof}


\kar{I don't see how to make this reduction linear.
\begin{lemma}
Given an alternating $\Val$-automaton of which the universality is history deterministic, deciding whether the nondeterminism is also history deterministic reduces to deciding the best value synthesis problem of a \textit{universal} $\Val$-automaton $\A'$.% Furthermore, the witness of history-determinism of $\A$ is implementable by the same computational models as the solution to the synthesis problem of $\A'$.
\end{lemma}
}
\kar{We need to go over this argument... with an alternating automaton, how do I put the transition in the letter? Essentially the output letter should store a local strategy.
\begin{proof}
$\A'$ be the $\Val$-automaton $(\Sigma \times 2^\Delta, Q,\iota,\delta')$
where $\delta'(q,(a,q\xrightarrow{a:x}q'))= \bigwedge_{c\in \delta(q,a)}$ if $(x,q')\in c$. $\A'$ maps valid runs of $\A$ written as pairs $(w,r)$ where $r$ is a run of $\A$ over $w$, onto $\Val(r)$ and in particular $\best{\A'}{I}=\A(I)$.
We claim that $\A'$ is best-value realisable if and only $\A$ is history-deterministic. Indeed,  a solution $s$ to the best value synthesis problem of $\A'$ corresponds to a function building a run of $\A$ over the input $I$ transition by transition such that the value of the run is $\best{\A'}{I}$. Since $\best{\A'}{I}$ is $\A(I)$, $s$ is precisely a witness of history-determinism in $\A$. Similarly, a witness of history-determinism in $\A$ induces a solution to the best value synthesis problem for $\A'$ since it builds a run of $\A$ over $I$ with value at least $\A(I)$, exactly what is required from a solution to the best value synthesis.
\end{proof}
}

\todo{In what level of detail do we want to talk about approximative synthesis and $r$-regret histroy-determinism?}

Using similar ideas, the approximative synthesis problem reduces to deciding a similarly parameterised notion of history determinism, known as $r$-regret GFGness~\cite{HPR15}, which, in some contexts, is equivalent to the $r$-regret determinisability as defined in~\cite{FLW20}. 
 
\subsection{Good-enough threshold synthesis}

While best value synthesis requires the system to match exactly the best possible value, the good-enough threshold synthesis problem only requires the system to guarantee a fixed threshold value, and only on inputs that are involved in some global behaviour with value of at least the threshold.

As the name suggests, the good-enough threshold synthesis problem is a quantitative generalisation of the good-enough synthesis problem of boolean automata~\cite{AK20}.


\begin{description}
\item[Input] Specification $f: (\Sigma_I \times \Sigma_O)^\omega \rightarrow \mathbb{R}$, threshold $t\in \mathbb{R}$
\item[System] Function $s:\Sigma^*_I \rightarrow \Sigma_O$ such that for all $I\in \Sigma_I^\omega$, if there exists $O\in \Sigma_O^\omega$ such that $f(I\otimes O)\geq t$ then $f(I\otimes \out{s}(I))\geq t$.
\item[Realisability] Does such a function $s$ [implementable with a memory $M$] exist?
\item[Synthesis] If yes, output an implementation with memory $M$ of $s$.
\end{description}

While solving best value synthesis reduces to deciding history-determinism, solving good-enough threshold synthesis with a threshold $t$ reduces to deciding \textit{$t$-threshold history determinism}, using similar reductions to the ones in the previous section.
 
 
\begin{lemma}
Deciding the good-enough $t$-threshold synthesis problem of a history-deterministic nonterministic $\Val$-automaton $\A$ reduces to deciding whether a nondeterministic $\Val$-automaton $\A'$ is $t$-threshold history-deterministic. 
\end{lemma}


The idea of the reducton is the same as above: the choice of output letter $\A$ turns into nondeterministic choices in $\A'$, the automaton that maps inputs $I\in \Sigma_I^\omega$ onto $\best{\A}{I}$. Then, a solution to the good-enough $t$-threshold synthesis problem for $\A$ corresponds exactly to a function that resolves the nondeterminism of $\A'$ on the fly while guaranteeing that for all inputs $I$ such that $\A'(I)\geq t$, the run built by the function has value at least $t$, in other words, this is exactly a witnesses of the $t$-threshold history-determinism of $\A'$. As above, $\A$ can itself be nondeterministic, as long as it is $t$-threshold history-deterministic since the witness of $\A$'s $t$-threshold history-determinism can be combined with the solution to the synthesis problem to create a witness the $t$-threshold history-determinism of $\A'$.

\todo{More formal proof for the appendix?}

\begin{lemma}
Deciding whether a nondeterministic $\Val$-automaton $\A$ is $t$-threshold history-deterministic reduces to deciding the good-enough $t$-threshold synthesis problem of a deterministic $\Val$-automaton $\A'$. Furthermore, the witness of history-determinism of $\A$ has the same memory requirements as the solution to the good enough $t$-threshold synthesis problem of $\A'$.
\end{lemma}


As in the previous section, we build a deterministic automaton $\A'$ that maps words $(w,\rho)$ where $\rho$ is a valid run of $\A$ over $w$ onto the value or $\rho$ in $\A$, so that $\best{\A'}{w}=\A(w)$. Then, a solution to the good enough $t$-threshold synthesis problem of $\A'$ has to build for each $w$ a run $\rho$ of $\A$ such that $\Val(\rho)\geq t$ if $\A(w)\geq t$, i.e it corresponds exactly to a witness of $t$-threshold history-determinism for $\A$.


\kar{More details?}
\subsection{Value Synthesis}

Both of the previous two synthesis problems ask a decision question -- is a specification realisable? -- and ask for an implementation of the solution when it exists. In other words, they ask whether a reactive system's performance can match the theoretical maximum (or exceed a threshold) as prescribed by the specification.
The value synthesis on the other hand simply asks what is the best that the reactive system can guarantee~\cite{RCHJ09, CHJS11}. 

\begin{description}
\item[Input] A specification $f: (\Sigma_I \times \Sigma_O)^\omega \rightarrow \mathbb{R}$
\item[System] Function $s:\Sigma^*_I \rightarrow \Sigma_O$ has value $v$ if for all $I\in \Sigma_I^\omega$ we have $f(I\otimes \out{s}(I))\geq v$.
\item[Value] The maximal value $v$ of a function $s$ [implementable with a memory structure $M$]?
\item[Synthesis] Output implementation of $s$ with memory structure $M$ that guarantees the maximal value $v$.
\end{description}


Unlike best-value synthesis and good-enough synthesis, this version of the synthesis problem does not reduce to deciding history-determinism. Rather, just like for deterministic automata, solving the value synthesis problem of a function given by a good-for-games alternating $\Val$-automata $\A$ reduces to deciding the value of a $\Val$-game $G_\A$. Interestingly, if $\A$ is nondeterministic, then an optimal strategy in $G_\A$, implemented by some memory $M$, induces an optimal solution to the synthesis problem of $\A$ with the same memory $M$. However, if $\A$ is alternating, then the size of the optimal solution to the synthesis problem might be larger.
\kar{could we give an example of when this is infinite? That would be cool... Else where it's bigger would be nice too}

\begin{lemma}\label{lem:valuegfg}
Given a good-for-games $\Val$-alternating automaton $\A=(\Sigma_I\times \Sigma_O,Q,\iota,\delta)$, its synthesis value is the value of the $\Val$-game $G_\A=(Q,\iota,\delta')$ where $\delta'(q)=\bigwedge_{a\in \Sigma_I}\bigvee_{b\in \Sigma_O} \delta(q,(a,b))$.

In addition, if $\A$ is nondeterministic, then a strategy in $\G_\A$ induces a solution in the synthesis problem, potentially with $\G_\A$ as additional memory.

Finally, if $\A$ is alternating but the universality in $\A$ is history deterministic witnessed by $s$, then a strategy in $\G_\A$ combined with the strategy witnessing the history determinism of the universality in $\A$ induces a solution to the synthesis problem. 
\end{lemma}

\begin{proof}
The synthesis problem for $\A$ can be described as the $\A$-game $\G=(\{q\},\bigwedge_{a\in \Sigma_I}\bigvee_{b\in \Sigma_O} ((a,b),q)$ in which Adam and Eve alternatively pick letters and the payoff is given by $\A$. Then, since $\A$ is good-for-games, the product $\G\times \A$ has the same value as $\G$. However, $\G\times \A= (q\times Q, q\times \iota, \delta')$ where $\delta'(q,p)= (q, \bigwedge_{a\in \Sigma_I}\bigvee_{b\in \Sigma_O} \delta(p,(a,b))$, that is, by renaming states $(q,p)$ to $p$, exactly $\G_\A$.


If $\A$ is nondeterministic, then a strategy for Eve in $\G_\A$ induces a strategy in $\G$, that is, a solution to the synthesis problem: indeed, $\sigma_E$ can be seen as producing output letters, and building a run in $\G$ with value at least $v$, witnessing that the value of the play in $\G$ is at least $v$. 

However, if $\A$ is alternating, this is no longer the case, as the strategy $\sigma_E$ depends on the history of the play in $\G_\A$, and in particular on Adam's moves that resolve the universality in $\A$. Since in $\G$ Adam only plays input letters, $\sigma_E$ does not induce a strategy in $\G$. Indeed, is Eve uses an arbitrary choice to resolve the universal choices in $\A$, the produced run only shows that some run of $\A$ has value $v$, but it does not guarantee that Adam could not have achieved a lower value had he played differently from Eve's arbitrary choices.

However, if the universality of $\A$ is history deterministic with witness $s$, then $\sigma_E$, combined with $s$, induces a solution to the synthesis problem: indeed, $\sigma_E$ seen as a strategy in the game $\G_\A$ restricted to the plays compatible with $s$ produces for every input prefix an output letter and a run in $\A$ with value at least $v$ over the produced word $w$. Since this run is compatible with $s$, a witness of the history determinism of the universality of $\A$, this guarantees that the value of $w$ is not less than $v$, proving that this strategy is a solution to the synthesis problem. The implementation of this solution depends on both the complexity of the solution of $\G_\A$ and on the complexity of the witness of the history determinism of the universality of $\A$. 
\end{proof}

\subsection{Threshold synthesis}

Finally, the threshold synthesis problem asks whether the reactive system can guarantee the threshold in all environments, that is, whether the solution of the value synthesis problem exceeds the threshold.

\begin{description}
\item[Input] Specification $f: (\Sigma_I \times \Sigma_O)^\omega \rightarrow \mathbb{R}$, threshold $t$
\item[System] Function $s:\Sigma^*_I \rightarrow \Sigma_O$ has value $v$ if for all $I\in \Sigma_I^\omega$ we have $\Val(I\otimes \out{s}(I))\geq v$.
\item[Realisability] Is there a function $s$ [implemented by a memory $X$] with value at least $t$?
\item[Synthesis] Output $X$ that implements $s$ with value at least $t$.
\end{description}

We can use the same argument as in the previous section to reduce the $t$-threshold synthesis problem to solving a $t$-threshold game. However,  while above the reduction required the automaton to be good-for-games, here we only require the automaton to be good for $t$-threshold games for the fixed threshold $t$.


\begin{lemma}
The $t$-threshold synthesis problem of a good for $t$-threshold games $\Val$-alternating automaton $\A=(\Sigma_I\times \Sigma_O,Q,\iota,\delta)$, reduces to the $t$-threshold game $G_\A=(Q,\iota,\delta')$ where $\delta'(q)=\bigwedge_{a\in \Sigma_I}\bigvee_{b\in \Sigma_O} \delta(q,(a,b))$ with $\Val$ as payoff function.

In addition, if $\A$ is nondeterministic, then a strategy in $\G_\A$ induces a solution in the synthesis problem, with $\G_\A$ as additional memory.

Finally, if $\A$ is alternating but the universality in $\A$ is $t$-threshold history deterministic witnessed by $s$, then a strategy in $\G_\A$ combined with the strategy witnessing the history determinism of the universality in $\A$ induces a solution to the synthesis problem. 
\end{lemma}

The proof is again the same as for~\cref{lem:valuegfg}, but we only need $\A$ to be goof for $t$-threshold games. As before, the strategy in the product game can provide a solution in the original game, but only if the universality is $t$-threshold history deterministic, and in particular if $\A$ is nondeterministic.
